Language-integrated provenance

Provenance, or information about the origin or derivation of data, is important for assessing the trustworthiness of data and identifying and correcting mistakes. Most prior implementations of data provenance have involved heavyweight modifications to database systems and little attention has been paid to how the provenance data can be used outside such a system. We present extensions to the Links programming language that build on its support for language-integrated query to support provenance queries by rewriting and normalizing monadic comprehensions and extending the type system to distinguish provenance metadata from normal data. The main contribution of this article is to show that the two most common forms of provenance can be implemented efficiently and used safely as a programming language feature with no changes to the database system.

==> lineage_group_m.tex <==
% Created by tikzDevice version 0.10.1 on 2017-05-24 16:06:06
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (325.21,252.94);
\begin{scope}
\path[clip] ( 27.77,189.81) rectangle (325.21,240.88);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (108.64,192.13) rectangle (125.37,195.68);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] ( 91.90,192.71) rectangle (108.64,195.68);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] ( 75.17,195.68) rectangle ( 91.90,196.02);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] ( 58.44,194.12) rectangle ( 75.17,195.68);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] ( 41.71,195.68) rectangle ( 58.44,200.02);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (201.59,195.68) rectangle (218.32,202.03);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] (184.86,195.68) rectangle (201.59,206.48);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] (168.13,195.68) rectangle (184.86,206.82);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] (151.39,195.68) rectangle (168.13,205.78);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] (134.66,195.68) rectangle (151.39,207.58);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (294.54,195.68) rectangle (311.27,221.31);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] (277.81,195.68) rectangle (294.54,214.88);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] (261.08,195.68) rectangle (277.81,229.67);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] (244.35,195.68) rectangle (261.08,215.72);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] (227.62,195.68) rectangle (244.35,225.20);
\end{scope}
\begin{scope}
\path[clip] ( 27.77,107.45) rectangle (325.21,158.52);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (108.64,113.32) rectangle (125.37,115.01);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] ( 91.90,113.32) rectangle (108.64,116.38);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] ( 75.17,113.32) rectangle ( 91.90,117.50);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] ( 58.44,113.32) rectangle ( 75.17,116.16);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] ( 41.71,113.32) rectangle ( 58.44,129.36);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (201.59,113.32) rectangle (218.32,124.85);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] (184.86,113.32) rectangle (201.59,130.08);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] (168.13,113.32) rectangle (184.86,130.12);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] (151.39,113.32) rectangle (168.13,129.44);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] (134.66,113.32) rectangle (151.39,135.06);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (294.54,113.32) rectangle (311.27,141.70);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] (277.81,113.32) rectangle (294.54,146.41);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] (261.08,113.32) rectangle (277.81,151.30);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] (244.35,113.32) rectangle (261.08,141.68);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] (227.62,113.32) rectangle (244.35,152.74);
\end{scope}
\begin{scope}
\path[clip] ( 27.77, 25.09) rectangle (325.21, 76.16);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (108.64, 30.96) rectangle (125.37, 39.37);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] ( 91.90, 30.96) rectangle (108.64, 40.20);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] ( 75.17, 30.96) rectangle ( 91.90, 42.09);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] ( 58.44, 30.96) rectangle ( 75.17, 39.69);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] ( 41.71, 30.96) rectangle ( 58.44, 61.63);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (201.59, 30.96) rectangle (218.32, 50.60);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] (184.86, 30.96) rectangle (201.59, 51.19);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] (168.13, 30.96) rectangle (184.86, 51.37);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] (151.39, 30.96) rectangle (168.13, 50.97);
\definecolor{fillColor}{RGB}{0,0,0}

\path[fill=fillColor] (134.66, 30.96) rectangle (151.39, 64.56);
\definecolor{fillColor}{RGB}{240,228,66}

\path[fill=fillColor] (294.54, 30.96) rectangle (311.27, 68.22);
\definecolor{fillColor}{RGB}{0,158,115}

\path[fill=fillColor] (277.81, 30.96) rectangle (294.54, 70.78);
\definecolor{fillColor}{RGB}{86,180,233}

\path[fill=fillColor] (261.08, 30.96) rectangle (277.81, 73.84);
\definecolor{fillColor}{RGB}{230,159,0}

\path[fill=fillColor] (244.35, 30.96) rectangle (261.08, 69.80);
\end{scope}
\begin{scope}
\path[clip] ( 27.77, 76.16) rectangle (325.21, 93.23);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (176.49, 81.66) {64};
\end{scope}
\begin{scope}
\path[clip] ( 27.77,158.52) rectangle (325.21,175.59);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (176.49,164.02) {32};
\end{scope}
\begin{scope}
\path[clip] ( 27.77,240.88) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (176.49,246.38) {16};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 83.54, 22.34) --
	( 83.54, 25.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (176.49, 22.34) --
	(176.49, 25.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (269.44, 22.34) --
	(269.44, 25.09);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 83.54, 15.32) {10000};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (176.49, 15.32) {1e+05};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (269.44, 15.32) {1e+06};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.50] at ( 22.82,208.68) {10};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.50] at ( 22.82,238.13) {1000};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.02,210.41) --
	( 27.77,210.41);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.02,239.85) --
	( 27.77,239.85);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.50] at ( 22.82,126.32) {10};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.50] at ( 22.82,155.77) {1000};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.02,128.05) --
	( 27.77,128.05);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.02,157.49) --
	( 27.77,157.49);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.50] at ( 22.82, 43.96) {10};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.50] at ( 22.82, 73.41) {1000};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.02, 45.69) --
	( 27.77, 45.69);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.02, 75.13) --
	( 27.77, 75.13);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (176.49,  5.00) {rows};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,252.94);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (  4.82,132.99) {Time (s)};
\end{scope}
\end{tikzpicture}

